Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of summer 2016

This article reports world averages of measurements of $b$-hadron, $c$-hadron, and $\tau$-lepton properties obtained by the Heavy Flavor Averaging Group using results available through summer 2016. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, \CP~violation parameters, parameters of semileptonic decays and CKM matrix elements.

==> b2charm/Bd_DD_11.tex <==
\begin{btocharmtab}{Bd_DD_11}{Product decay rates to excited $D_s$ mesons II $[10^{-4}]$}
\hline
\textbf{Parameter} & \begin{tabular}{l}\textbf{Measurements}\end{tabular} & \textbf{Average} \\
\hline
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{-} D^{+} )\times {\cal{B}} ( D_{s1}(2536)^{-} \to D^{*}(2010)^{-} \bar{K}^{0} )}$}\\
 & \begin{tabular}{l} \babar \cite{Aubert:2007rva}: $2.61 \pm 1.03 \pm 0.31$ \\ \end{tabular} & $2.61 \pm 1.08$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{-} D^{+} )\times {\cal{B}} ( D_{s1}(2536)^{-} \to K^{-} \bar{D}^{*}(2007)^{0} )}$}\\
 & \begin{tabular}{l} \babar \cite{Aubert:2007rva}: $1.71 \pm 0.48 \pm 0.32$ \\ \end{tabular} & $1.71 \pm 0.58$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{-} D^{*}(2010)^{+} )\times {\cal{B}} ( D_{s1}(2536)^{-} \to D^{*}(2010)^{-} \bar{K}^{0} )}$}\\
 & \begin{tabular}{l} \babar \cite{Aubert:2007rva}: $5.00 \pm 1.51 \pm 0.67$ \\ \end{tabular} & $5.00 \pm 1.65$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{-} D^{*}(2010)^{+} )\times {\cal{B}} ( D_{s1}(2536)^{-} \to \bar{D}^{*}(2007)^{0} K^{+} )}$}\\
 & \begin{tabular}{l} \babar \cite{Aubert:2007rva}: $3.32 \pm 0.88 \pm 0.66$ \\ \end{tabular} & $3.32 \pm 1.10$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{+} D^{-} )\times {\cal{B}} ( D_{s1}(2536)^{+} \to D^{*}(2007)^{0} K^{+} + D^{*}(2010)^{+} K^{0} )}$}\\
 & \begin{tabular}{l} Belle \cite{Belle:2011ad}: $2.75 \pm 0.62 \pm 0.36$ \\ \end{tabular} & $2.75 \pm 0.72$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{+} D^{*}(2010)^{-} )\times {\cal{B}} ( D_{s1}(2536)^{+} \to D^{*}(2007)^{0} K^{+} + D^{*}(2010)^{+} K^{0} )}$}\\
 & \begin{tabular}{l} Belle \cite{Belle:2011ad}: $5.01 \pm 1.21 \pm 0.70$ \\ \end{tabular} & $5.01 \pm 1.40$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D_{s1}(2536)^{+} D^{*}(2010)^{-} )\times {\cal{B}} ( D_{s1}(2536)^{+} \to D^{*}(2010)^{+} K_S^{0} )}$}\\
 & \begin{tabular}{l} Belle \cite{Dalseno:2007hx}: $< 6.0$ \\ \end{tabular} & $< 6.0$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D^{+} D_{sJ}(2460)^{-} )\times {\cal{B}} ( D_{sJ}(2460)^{-} \to D_s^{-} \pi^{+} \pi^{-} )}$}\\
 & \begin{tabular}{l} Belle \cite{Krokovny:2003zq}: $< 2.0$ \\ \end{tabular} & $< 2.0$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D^{+} D_{sJ}(2460)^{-} )\times {\cal{B}} ( D_{sJ}(2460)^{-} \to D_s^{-} \pi^{0} )}$}\\
 & \begin{tabular}{l} Belle \cite{Krokovny:2003zq}: $< 3.6$ \\ \end{tabular} & $< 3.6$ \\
\hline
\multicolumn{3}{|l|}{${{\cal{B}} ( \bar{B}^{0} \to D^{+} D_{sJ}(2460)^{-} )\times {\cal{B}} ( D_{sJ}(2460)^{-} \to D_s^{*-} \gamma )}$}\\
 & \begin{tabular}{l} Belle \cite{Krokovny:2003zq}: $< 6.0$ \\ \end{tabular} & $< 6.0$ \\
\hline
\end{btocharmtab}
\btocharmfig{Bd_DD_11}


==> b2charm/Bu_cc_12.tex <==
\begin{btocharmtab}{Bu_cc_12}{Direct \CP\ violation parameters}
\hline
\textbf{Parameter} & \begin{tabular}{l}\textbf{Measurements}\end{tabular} & \textbf{Average} \\
\hline
\hline
$A_{\CP} ( B^{-} \to J/\psi K^{-} )$ & \begin{tabular}{l} \dzero \cite{Abazov:2013sqa}: $0.0059 \pm 0.0036 \pm 0.0007$ \\ \end{tabular} & $0.0059 \pm 0.0037$ \\
\hline
$A_{\CP} ( B^{-} \to J/\psi \pi^{-} )$ & \begin{tabular}{l} \dzero \cite{Abazov:2013sqa}: $-0.042 \pm 0.044 \pm 0.009$ \\ \end{tabular} & $-0.042 \pm 0.045$ \\
\hline
\end{btocharmtab}
\btocharmfig{Bu_cc_12}


==> tables/slb/pilnubf.tex <==
\begin{sidewaystable}[!htb]
\begin{center}
\caption{\label{tab:pilnubf}
Summary of exclusive determinations of $\cbf(\Bb\to\pi
\ell\nub)$. The errors quoted
correspond to statistical and systematic uncertainties, respectively.
Measured branching fractions for $B^+\rightarrow \pi^0 \ell^+ \nu$ have been
multiplied by $2\times \tau_{B^0}/\tau_{B^+}$ in accordance with
isospin symmetry. The labels ``had. tag'' and ``sl. tag'' refer to
the type of $B$ tag used in the measurement, and ``untagged'' refers to an untagged measurement.}
\begin{small}
\begin{tabular}{|lcccc|}
\hline
& $\cbf [10^{-4}]$
& $\cbf(q^2<12\,\gev^2/c^2) [10^{-4}]$
& $\cbf(q^2<16\,\gev^2/c^2) [10^{-4}]$
& $\cbf(q^2>16\,\gev^2/c^2) [10^{-4}]$
\\
\hline\hline
CLEO untagged $\pi^+,\pi^0$~\cite{Adam:2007pv}
& $1.38\pm 0.15\pm 0.11$ 
& $0.69\pm 0.12\pm 0.07$
& $0.97\pm 0.13\pm 0.09$
& $0.41\pm 0.08\pm 0.04$
\\ 
\babar untagged $\pi^+,\pi^0$~\cite{delAmoSanchez:2010af}
& $1.41\pm 0.05\pm 0.08$
& $0.88\pm 0.04\pm 0.05$
& $1.10\pm 0.04\pm 0.06$
& $0.32\pm 0.02\pm 0.03$
\\  
\babar untagged $\pi^+, \pi^0$~\cite{Lees:2012vv}
& $1.44\pm 0.04\pm 0.06$
& $0.83\pm 0.03\pm 0.04$
& $1.08\pm 0.03\pm 0.05$
& $0.40\pm 0.02\pm 0.02$
\\  
Belle untagged $\pi^+$~\cite{Ha:2010rf}
& $1.48\pm 0.04\pm 0.07$
& $0.82\pm 0.03\pm 0.04$
& $1.09\pm 0.03\pm 0.05$
& $0.40\pm 0.02\pm 0.02$
\\  
Belle sl. tag $\pi^+$~\cite{Hokuue:2006nr}
& $1.41\pm 0.19\pm 0.15$
& $0.80\pm 0.14\pm 0.08$
& $1.04\pm 0.16\pm 0.11$
& $0.37\pm 0.10\pm 0.04$
\\ 
Belle sl. tag $\pi^0$~\cite{Hokuue:2006nr}
& $1.41\pm 0.26\pm 0.15$
& $0.71\pm 0.17\pm 0.08$
& $1.05\pm 0.22\pm 0.12$
& $0.37\pm 0.15\pm 0.04$
\\ 
\babar sl. tag $\pi^+$~\cite{Aubert:2008bf}
& $1.38\pm 0.21\pm 0.08$
& $0.77\pm 0.14\pm 0.05$
& $0.92\pm 0.16\pm 0.05$
& $0.46\pm 0.13\pm 0.03$
\\ 
\babar sl. tag $\pi^0$~\cite{Aubert:2008bf}
& $1.78\pm 0.28\pm 0.15$
& $1.07\pm 0.20\pm 0.09$
& $1.35\pm 0.22\pm 0.11$
& $0.44\pm 0.17\pm 0.06$
\\ 
\babar had. tag $\pi^+$~\cite{Aubert:2006ry}
& $1.07\pm 0.27\pm 0.19$
& $0.26\pm 0.15\pm 0.04$
& $0.42\pm 0.18\pm 0.06$
& $0.65\pm 0.20\pm 0.13$
\\ 
\babar had. tag $\pi^0$~\cite{Aubert:2006ry}
& $1.52\pm 0.41 \pm0.30$
& $0.67\pm 0.30\pm 0.12$
& $1.04\pm 0.35\pm 0.18$
& $0.48\pm 0.22\pm 0.12$
\\ 
Belle had. tag $\pi^+$~\cite{Sibidanov:2013rkk}
& $1.49\pm 0.09\pm 0.07$
& $0.81\pm 0.06\pm 0.04$
& $1.06\pm 0.07\pm 0.05$
& $0.45\pm 0.05\pm 0.02$
\\ 
Belle had. tag $\pi^0$~\cite{Sibidanov:2013rkk}
& $1.48\pm 0.15\pm 0.08$
& $0.78\pm 0.11\pm 0.04$
& $1.09\pm 0.12\pm 0.06$
& $0.36\pm 0.07\pm 0.02$
\\  \hline
{\bf Average}
& \mathversion{bold}$1.45\pm 0.02\pm 0.04$
& \mathversion{bold}$0.81\pm 0.02\pm 0.02$
& \mathversion{bold}$1.06\pm 0.02\pm 0.03$
& \mathversion{bold}$0.38\pm 0.01\pm 0.01$
\\ 
\hline
\end{tabular}\\
\end{small}
\end{center}
\end{sidewaystable}


==> tables/slb/pilnuvub.tex <==

\begin{table}[hbt]
\caption{\label{tab:pilnuvub}
Determinations of \vub\ based on the average partial
$\Bb\to\pi\ell\nub$ decay branching fractions stated in
Table~\ref{tab:pilnubf}. 
The $q^2$ ranges for the partial branching fractions corresponding to the 
validity ranges of the form factor calculations are indicated. 
The first uncertainty is experimental and the second is from theory.  
}
%\scriptsize
%\vspace{5mm} 
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|lcc|}
\hline
Method                                         & $q^2$ range [$\gev^2/c^2$] & $\Vub [10^{-3}]$ \\\hline\hline
Khodjamirian et al. (LCSR) ~\cite{Khodjamirian:2011ub} & 0 -- 12                    & $3.41\pm 0.06 {}^{+0.37}_{-0.32}$ \\ \hline
Ball \& Zwicky (LCSR)~\cite{Ball:2004ye}              & 0 -- 16                    & $3.58\pm 0.06 {}^{+0.59}_{-0.40}$ \\ \hline
HPQCD (LQCD)~\cite{Dalgic:2006dt}                     & 16 -- 26.4                 & $3.52\pm 0.08 {}^{+0.61}_{-0.40}$ \\  \hline
FNAL/MILC (LQCD)~\cite{Bailey:2008wp}                 & 16 -- 26.4                 & $3.36\pm 0.08 {}^{+0.37}_{-0.31}$ \\ 
%APE, $q^2>16\,\gev^2/c^2$~\cite{Abada:2000ty}         & $3.72\pm 0.21 {}^{+1.43}_{-0.66}$ \\ 
\hline
\end{tabular}
\end{center}
\end{table}


==> tau/tau-br-fit-meas-byref.tex <==
%% ///////////////////////////////////////////////////////////////////////////
%%\appendix
\tausection{Branching fractions fit measurement list by reference}
\cutname{br-fit-meas-byref.html}

Table~\ref{tab:tau:measPerPaper} reports the measurements used for the
\hfagtau branching fraction fit grouped by their bibliographic reference.

%%
%% By-reference measurements list
%%
\begin{center}
\begin{envsmall}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{longtable}{ll}
\caption{By-reference measurements list.\label{tab:tau:measPerPaper}}%
\\
\hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endfirsthead
\multicolumn{2}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endhead
\htuse{MeasPaper} \\
\hline
\end{longtable}
\end{envsmall}
\end{center}

